Stock-driven Household Attention

We investigate the effects of stockholding on households' attention to the macroeconomy. Households' attentiveness is measured by their accuracy of inflation expectations and perceptions. Relative to non-stockholders, stockholders produce more accurate inflation forecasts and backcasts, disagree less about future inflation, and adjust their outlook more responsively to news, suggesting that stock-market participation raises households' attention. Frequent changes in stock prices incentivize stockholders to closely monitor financial markets for optimal trading, given the low cost of acquiring information. Consequently, paying attention to the macroeconomy helps hedge the risks associated with holding stocks. Therefore, attention heterogeneity driven by stockholdings can be a channel through which the distributional consequences of monetary policy are created.

==> Archive/Gasoline.tex <==
"What does the county-level gasoline prices tell us about households' expectations on gasoline price changes?"

I think this is an important question... Here are two materials that may help us to think through the problem. 

- Why Gas Prices Are So High in California - The New York Times (nytimes.com)

- Davis, Michael C & Hamilton, James D, 2004. "Why Are Prices Sticky? The Dynamics of Wholesale Gasoline Prices," Journal of Money, Credit and Banking, Blackwell Publishing, vol. 36(1), pages 17-37, February.

Stuck in the Seventies: Gas Prices and Consumer Sentiment

https://direct.mit.edu/rest/article-abstract/104/2/293/97647/Stuck-in-the-Seventies-Gas-Prices-and-Consumer?redirectedFrom=fulltext

They used cross-sectional variations in gas prices in this paper.

==> Archive/ToDoList_Nov22.tex <==



Here is the recap of our meeting just to keep track of what we discussed and our homework. (November 15th 2022)

1. HJ 
-- [1] Priority: write a paper throughout except for the theory part. 
-- [2] Michigan nowcast -- linking nowcast to forecast -- Kalman gain update + information rigidity (will reach out to shihan for more discussion)


2. Shihan
-- [1] Table 4 : remove Panel A from the table and move it to the appendix? 
-- [2] HJ : will write a story that there is some evidence that the information shocks are informative of future inflation, but the evidence is inconclusive. This may be due to the measurement issues in the information shock which is the actively debated and researched area these days. 


3. Choong
-- [1] work on theory -- stock-holders and hand-to-mouth individuals 
-- [2] mentioned counter-cyclical attention : established relationship between uncertainty and attention ; consistent with what we are thinking. 
-- [3] mentioned individual-level uncertainty and durable-goods consumption (menu-cost type of behavior) --  Geng Li has a paper about it. 
-- [4] HJ : Notice that individual-level uncertainty affects job-search behavior differently. Perhaps we can establish some stylized facts about how individual-level uncertainty affects an individual's forward-looking behavior or economic activities (we can distinguish production side and consumption side)

==> LitReviewText.tex <==

Limited Stock Market Participation Among Renters and Homeowners (Vestman, Roine)

The stock market participation rate among homeowners is twice as high as among renters. This paper builds a life-cycle portfolio choice model with endogenous housing tenure choice. A stylized form of preference heterogeneity generates a substantial difference in participation rates. A majority of households have a large savings motive and choose to be homeowners and participate. A minority of households have a small savings motive and find it less worthwhile to participate. Fewer of these households become homeowners. Difference-in-difference regressions on panel data do not find evidence of a crowding-out effect of homeownership on participation, supporting the message that preference heterogeneity matters.


Socioeconomic Status and Macroeconomic Expectations (Das, Sreyoshi and Kuhnen, Camelia M and Nagel, Stefan)

We show that individuals’ macroeconomic expectations are influenced by their socioeconomic status (SES). People with higher income or higher education are more optimistic about future macroeconomic developments, including business conditions, the national unemployment rate, and stock market returns. The spread in beliefs between high- and low-SES individuals diminishes significantly during recessions. A comparison with professional forecasters and historical data reveals that the beliefs wedge reflects excessive pessimism on the part of low-SES individuals. SES-driven expectations help explain why higher-SES individuals are more inclined to invest in the stock market and more likely to consider purchasing homes, durable goods, or cars.

Consumers' Attitudes and Their Inflation Expectations (Michael Ehrmanna, Damjan Pfajfarb and Emiliano Santoro)

This paper studies consumers' inflation expectations using micro-level data from the University of Michigan's Surveys of Consumers. It shows that beyond the well-established socioeconomic factors such as income, age, or gender, inflation expectations are also related to respondents' financial situation, their purchasing attitudes, and their expectations about the macroeconomy. Respondents with current or expected financial difficulties and those with pessimistic attitudes about major purchases, income developments, or unemployment have a stronger upward bias than other households. However, their bias shrinks by more than that of the average household in response to increasing media reporting about inflation.


Rational Inattention in Uncertain Business Cycles (FANG ZHANG)

The paper proposes endogenous information choice as a channel through which uncertainty affects price dynamics. I consider a rational inattention model with volatility uncertainty and endogenous information processing capability. According to the model, firms' learning and optimal attention exhibits inertia and asymmetry in response to volatility changes. Firms choose to process more information when uncertainty rises, especially about aggregate conditions, and their pricing behavior changes accordingly. Using a Markov-switching factor-augmented vector autoregression (MS-FAVAR), the paper also documents a significant positive correlation between volatility and firms' responsiveness to macro- and microlevel shocks, consistent with model predictions.

Rational inattention to news: The perils of forward guidance (Gaetano Gaballo)

This paper studies the social value of information about the future. In a stylized OLG model, agents need to forecast the future price level, they observe the current price and perceive with idiosyncratic noise the expectation announced by a more informed authority. When forward guidance communication is loose, the market becomes a main source of information about the future. Reliance on market information amplifies the impact of shocks on prices, which increases ex ante uncertainty and worsens agents' forecasting ability, harming social welfare. However, an appropriate policy can convert the perils of the announcement in opportunities. 


Rational Inattention and Portfolio Selection (LIXIN HUANG and HONG LIU)

Costly information acquisition makes it rational for investors to obtain important economic news only with limited frequency or limited accuracy. We show that this rational inattention to important news may make investors overinvest or underinvest. In addition, the optimal trading strategy is “myopic” with respect to future news frequency and news accuracy. We find that the optimal news frequency is nonmonotonic in news accuracy and investment horizon. Furthermore, when both news frequency and news accuracy are endogenized, an investor with a higher risk aversion or a longer investment horizon chooses less frequent but more accurate periodic news updates.


Who Cares about Inflation? Endogenous Expectation Formation of Heterogeneous Households --Lukas Nord

This paper builds a joint theory of endogenous inflation expectations and consumption-savings choices of heterogeneous households. We introduce imperfect information about future inflation rates in a consumption-savings model and allow households to exert costly effort to reduce uncertainty about future price changes. High wealth households are more exposed to future inflation due to its effect on real interest rates and hence choose to be better informed. The joint distribution of wealth and inflation expectations generated by the model is consistent with key features of the data. The implied consumption response to news about inflation is hump shaped in wealth: Wealthier households pay closer attention and update their expectations more in response to any signal received, but change their consumption less after any given update in expectations due to the income effect of future inflation. We show this mechanism to reduce the on-impact aggregate consumption response to forward guidance policies by up to 55\% compared to an attentive counterfactual.


Inflation Expectations and Households Portfolio Choice -- Qingyuan Yang

Do household inflation expectations affect portfolio choice? This paper exploits inflation experience as an instrumental variable for inflation expectations and links it to household portfolios. I document that households with higher inflation expectations are more likely to invest in equity markets, shifting from safe assets to risky ones. Households can also achieve substantial financial returns and optimize their portfolio. I also document that households’ heterogeneous characteristics also contribute to the portfolio re-balance. In addition. I attribute the above findings to the income expectations and nominal rigidity of the deposit rate. These results imply households’ portfolio balancing behavior in response to increased inflation expectations.


==> Tables/summary_stat.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cccccc}}
\hline\hline
                    % &\multicolumn{6}{c}{(1)}                                                      \\
                    % &\multicolumn{6}{c}{}                                                         \\
                    &       count&        mean&          sd&         p75&         p50&         p25\\
\hline
1-year ahead inflation expectations&      124401&        3.41&        3.94&        5.00&        3.00&        1.00\\
1-year ahead gas price expectations&       83033&       16.09&       27.03&       25.00&        6.00&        0.00\\
Inflation forecast error&      124401&       -1.32&        4.17&        1.15&       -0.77&       -2.98\\
Gas price forecast error&       83033&      -16.43&       34.74&        6.95&       -9.14&      -36.47\\
\hline\hline
\end{tabular}
}


==> Tables/tab_attention.tex <==
\begin{table}
    \centering
    \caption{Stock holding, attention and attitudes towards the macroeconomy} \label{tab:attention}
    \small
    \centering
    \vspace{0.3cm}
	\noindent\resizebox{1.0\textwidth}{!}{
	\begin{tabularx}{\textwidth}{ll>{\centering}p{1.5cm}>{\centering}p{1.5cm}>{\centering}p{1.5cm}>{\centering}p{1.5cm}>{\centering}p{1.5cm}>{\centering}p{1.5cm}}
        \hline\hline
        \noalign{\vskip0.1cm}
         Dependent variable  & & \multicolumn{2}{c}{\textbf{Attentiveness}}   & \multicolumn{2}{c}{\textbf{Attitude}} & \multicolumn{2}{c}{\textbf{Sentiment}} \tabularnewline
         &  & (1) OLS & (2) IV & (3) OLS & (4) IV & (5) OLS & (6) IV \tabularnewline[0.1cm]
        \hline 
    	\noalign{\vskip0.1cm}
        Stock ($\beta$)  & &  0.08$^{***}$ &  0.10$^{***}$  &   0.02$^{***}$  & 0.03$^{**}$ & 3.86$^{***}$ & 5.30$^{***}$ \tabularnewline
                    & &     (0.00)          & (0.01)        &  (0.00)           & (0.01)   & (0.26)  & (0.69)        \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        Time FE          & & Y & Y & Y & Y & Y & Y  \tabularnewline[0.1cm]
        Demographics FE  & & Y & Y & Y & Y & Y & Y     \tabularnewline[0.1cm]
        Number of obs.  & & 120,147  &  45,987  & 120,147   & 45,987 & 120,147  &  45,987      \tabularnewline[0.1cm]
        $R^2$           & & 0.1045   &  0.0038   &   0.0784  & 0.0001 &  0.1755 & 0.0017   \tabularnewline[0.1cm]
        \hline\hline
        
    	\noalign{\vskip0.1cm}
    	\multicolumn{8}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Notes:} This table reports the regression results from Equations (\ref{eqn:error}). Dependent variables are \emph{Attentiveness} (Columns 1 and 2), \emph{Attitude} (Columns 3 and 4), and \emph{Sentiment} (Columns 5 and 6). "Stock" indicates dummies for stock market participation. We control for time-fixed effects and survey respondents' demographic fixed effects, including gender, education, birth cohort, marriage status, region, homeownership, and income quintiles. Columns (2), (4), and (6) use households' stock holding positions from six months ago as an instrument for current stock holding. Robust standard errors are reported in the parenthesis.  $^{***}$, $^{**}$, $^{*}$ denotes statistical significance at 1\%, 5\%, and 10\% levels respectively.}    \\ 
    	{\footnotesize \textit{Sources:} Authors' calculation.} 
	\end{tabularx}
    }
\end{table}

==> Tables/tab_control_attitude.tex <==
\begin{table}
    \centering
    \caption{Control for attitudes and sentiments} \label{tab:attention_control}
    \small
    \centering
    \vspace{0.3cm}
	\noindent\resizebox{1.0\textwidth}{!}{
	\begin{tabularx}{\textwidth}{ll>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}}
        \hline\hline
        \noalign{\vskip0.1cm}
         Dependent variable  & & \multicolumn{2}{c}{\textbf{Inflation}} & \multicolumn{2}{c}{\textbf{Gas price}} & \multicolumn{2}{c}{\textbf{Attentiveness}}   \tabularnewline 
         &  & (1) & (2) & (3) & (4) & (5) & (6) \tabularnewline[0.1cm]
        \hline 
    	\noalign{\vskip0.1cm}
        Stock ($\beta$)  & &  -0.345$^{***}$ &  -0.309$^{***}$  &   0.077  & 0.216 & 0.078$^{***}$ & 0.079$^{***}$ \tabularnewline
                    & &     (0.023)          & (0.023)        &  (0.135)   & (0.135)   & (0.003)  & (0.003)        \tabularnewline[0.1cm]
        Attitude    & & -0.344$^{***}$ & & -1.218$^{***}$ & & -0.119$^{***}$ \tabularnewline
                    & &  (0.012)        & & (0.074) & &  (0.002) \tabularnewline[0.1cm]
        Sentiment    & &        & -0.011$^{***}$  &  & -0.040$^{***}$ & & -0.001$^{***}$ \tabularnewline
                    & &         &  (0.000) & &  (0.001) & & (0.000) \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        Time FE          & & Y & Y & Y & Y & Y & Y  \tabularnewline[0.1cm]
        Demographics FE  & & Y & Y & Y & Y & Y & Y     \tabularnewline[0.1cm]
        Number of obs.  & & 108,026  &  108,026  & 67,460   & 67,460 & 120,147  &  120,147      \tabularnewline[0.1cm]
        $R^2$           & & 0.1255   &  0.1373   &   0.5475  & 0.5511 &  0.1305 & 0.1046   \tabularnewline[0.1cm]
        \hline\hline
        
    	\noalign{\vskip0.1cm}
    	\multicolumn{8}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Notes:} This table reports the regression results from Equations (\ref{eqn:error}) while controlling for attitudes and sentiments. Dependent variables are inflation forecast errors (Columns (1)-(2)), gas price forecast errors (Columns (3)-(4)), and attentiveness (Columns (5)-(6)) respectively. ``Stock'' indicates dummies for stock market participation. We control for time-fixed effects and survey respondents' demographic fixed effects, including gender, education, birth cohort, marriage status, region, homeownership, and income quintiles. Robust standard errors are reported in the parenthesis.  $^{***}$, $^{**}$, $^{*}$ denotes statistical significance at 1\%, 5\%, and 10\% levels respectively.}    \\ 
    	\multicolumn{8}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Sources:} Authors' calculation.} 
	\end{tabularx}
    }
\end{table}

==> Tables/tab_error.tex <==
\begin{table}
    \centering
    \caption{Stock holding and nowcast/forecast errors} \label{tab:error}
    \small
    \centering
    \vspace{0.3cm}
	\noindent\resizebox{1.0\textwidth}{!}{
	\begin{tabularx}{\textwidth}{ll>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}}
        \hline\hline
        \noalign{\vskip0.1cm}
         Dependent variable  & & \multicolumn{2}{c}{\textbf{Inflation}} & \multicolumn{2}{c}{\textbf{Gas price}} & \multicolumn{2}{c}{\textbf{Attentiveness}}   \tabularnewline
        &  & (1) OLS & (2) IV & (3) OLS & (4) IV & (5) OLS & (6) IV \tabularnewline[0.1cm]
        \hline 
    	\noalign{\vskip0.1cm}
        Stock ($\beta$)  &  & -0.371$^{***}$ & -0.595$^{***}$ &   0.181 &  0.181 & 0.08$^{***}$ &  0.10$^{***}$\tabularnewline
                    &   &    (0.024) & (0.061)  &    (0.115)  &    (0.347) & (0.00)          & (0.01) \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        Time FE          & & Y & Y & Y & Y & Y & Y  \tabularnewline[0.1cm]
        Demographics FE  & & Y & Y & Y & Y & Y & Y     \tabularnewline[0.1cm]
        %Sample period   & &  \multicolumn{2}{c}{2016 - 2021}    & \multicolumn{2}{c}{1997 - 2021} & \multicolumn{2}{c}{1997 - 2021} \tabularnewline[0.1cm]
        Number of obs.  &  &      109,001   & 42,404  &   64,492  &   26,980 & 120,147  &  45,987 \tabularnewline[0.1cm]
        $R^2$           &   &    0.1157   & 0.0011 &  0.2866   & -0.0001 & 0.1045   &  0.0038 \tabularnewline[0.1cm]
        \hline\hline
        
    	\noalign{\vskip0.1cm}
    	\multicolumn{8}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Notes:} This table reports the regression results from Equations (\ref{eqn:error}). Dependent variables are inflation forecast errors (Columns (1)-(2)), gas price forecast errors (Columns (3)-(4)), and attentiveness (Columns (5)-(6)) respectively. ``Stock'' indicates dummies for stock market participation. We control for time-fixed effects and survey respondents' demographic fixed effects, including gender, education, birth cohort, marriage status, region, homeownership, and income quintiles. Robust standard errors are reported in the parenthesis.  $^{***}$, $^{**}$, $^{*}$ denotes statistical significance at 1\%, 5\%, and 10\% levels respectively.}    \\ 
    	\multicolumn{8}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Sources:} Authors' calculation.} 
	\end{tabularx}
    }
\end{table}

==> Tables/tab_error_gasoline.tex <==
\begin{table}
    \centering
    \caption{Stock holding and gas price forecast errors} \label{tab:error_gasoline}
    \small
    \centering
    \vspace{0.3cm}
	\noindent\resizebox{1.0\textwidth}{!}{
	\begin{tabularx}{\textwidth}{ll>{\centering}p{5cm}>{\centering}p{5cm}}
        \hline\hline
        \noalign{\vskip0.1cm}
         Dependent variable  & & \multicolumn{1}{c}{\textbf{Gas price}}  \tabularnewline
        &  & (1) OLS & (2) IV  \tabularnewline[0.1cm]
        \hline 
        \noalign{\vskip0.1cm}
        Stock ($\beta$)  &  &   0.181 &  0.181 \tabularnewline
                    &   &   (0.115)  &    (0.347)  \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        Time FE          & & Y & Y  \tabularnewline[0.1cm]
        Demographics FE  & & Y & Y     \tabularnewline[0.1cm]
        %Sample period   & &  \multicolumn{2}{c}{2016 - 2021}    & \multicolumn{2}{c}{1997 - 2021} & \multicolumn{2}{c}{1997 - 2021} \tabularnewline[0.1cm]
        Number of obs.  &  &     64,492  &   26,980  \tabularnewline[0.1cm]
        $R^2$           &   &    0.2866   & -0.0001  \tabularnewline[0.1cm]
        \hline\hline
        
    	\noalign{\vskip0.1cm}
    \multicolumn{4}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Notes:} This table reports the regression results from Equations (\ref{eqn:error}). The dependent variable is gas price forecast errors (Columns (1)-(2)). ``Stock'' indicates dummies for stock market participation. We control for time-fixed effects and survey respondents' demographic fixed effects, including gender, education, birth cohort, marriage status, region, homeownership, and income quintiles. Robust standard errors are reported in the parenthesis.  $^{***}$, $^{**}$, $^{*}$ denotes statistical significance at 1\%, 5\%, and 10\% levels respectively.}    \\ 
    \multicolumn{4}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Sources:} Authors' calculation.} 
 \end{tabularx}
    }
\end{table}

==> Tables/tab_error_old.tex <==
\begin{table}
    \centering
    \caption{Stock holding and nowcast/forecast errors} \label{tab:error}
    \small
    \centering
    \vspace{0.3cm}
	\noindent\resizebox{1.0\textwidth}{!}{
	\begin{tabularx}{\textwidth}{ll>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}>{\centering}p{1.7cm}}
        \hline\hline
        \noalign{\vskip0.1cm}
                        & & \multicolumn{2}{c}{\textbf{Nowcast error}}   & \multicolumn{4}{c}{\textbf{Forecast error}} \tabularnewline
        Dependent variable &  &  \multicolumn{2}{c}{ Inflation} & \multicolumn{2}{c}{ Inflation} & \multicolumn{2}{c}{ Gas prices} \tabularnewline
        &  & (1) OLS & (2) IV & (3) OLS & (4) IV & (5) OLS & (6) IV \tabularnewline[0.1cm]
        \hline 
    	\noalign{\vskip0.1cm}
        Stock ($\beta$)  & & -1.002$^{***}$  &   & -0.371$^{***}$ & -0.595$^{***}$ &   0.181 &  0.181 \tabularnewline
                    & & (0.137)     &       &    (0.024) & (0.061)  &    (0.115)  &    (0.347) \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        Time FE          & & Y & Y & Y & Y & Y & Y  \tabularnewline[0.1cm]
        Demographics FE  & & Y & Y & Y & Y & Y & Y     \tabularnewline[0.1cm]
        Sample period   & &  \multicolumn{2}{c}{2016 - 2021}    & \multicolumn{2}{c}{1997 - 2021} & \multicolumn{2}{c}{1997 - 2021} \tabularnewline[0.1cm]
        Number of obs.  & & 13,624   &  &      109,001   & 42,404  &   64,492  &   26,980 \tabularnewline[0.1cm]
        $R^2$           & & 0.1031    &    &    0.1157   & 0.0011 &  0.2866   & -0.0001 \tabularnewline[0.1cm]
        \hline\hline
        
    	\noalign{\vskip0.1cm}
    	\multicolumn{8}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Notes:} This table reports the regression results from Equations (\ref{eqn:error}). Dependent variables are the inflation nowcast errors (Columns (1-2)), the inflation forecast errors (Columns (3-4)), and the gas price forecast errors (Columns (5-6)). "Stock" indicates dummies for stock market participation. We control for time-fixed effects and survey respondents' demographic fixed effects, including gender, education, birth cohort, marriage status, region, homeownership, and income quintiles. Robust standard errors are reported in the parenthesis.  $^{***}$, $^{**}$, $^{*}$ denotes statistical significance at 1\%, 5\%, and 10\% levels respectively.}    \\ 
    	\multicolumn{8}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Sources:} Authors' calculation.} 
	\end{tabularx}
    }
\end{table}

==> Tables/tab_error_old0.tex <==
\begin{table}[t]
    \centering
    \caption{Stock holding and nowcast/forecast errors} \label{tab:error}
    \small
    \centering
    \vspace{0.3cm}
	\noindent\resizebox{1.0\textwidth}{!}{
	\begin{tabularx}{\textwidth}{ll>{\centering}p{3.5cm}>{\centering}p{3.5cm}>{\centering}p{3.5cm}}
        \hline\hline
        \noalign{\vskip0.1cm}
                        & & \multicolumn{1}{c}{\textbf{Nowcast error}}   & \multicolumn{2}{c}{\textbf{Forecast error}} \tabularnewline
        Dependent variable &  & (1) Inflation & (2) Inflation & (3) Gas prices \tabularnewline[0.1cm]
        \hline 
    	\noalign{\vskip0.1cm}
        Stock ($\beta$)  & & -1.002$^{***}$  &  -0.371$^{***}$  &   0.181   \tabularnewline
                    & & (0.137)            &    (0.024)         &    (0.115)          \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        Time FE          & & Y & Y & Y  \tabularnewline[0.1cm]
        Demographics FE  & & Y & Y & Y      \tabularnewline[0.1cm]
        Sample period   & &  2016 - 2021    & 1997 - 2021 & 1997 - 2021 \tabularnewline[0.1cm]
        Number of obs.  & & 13,624     &      109,001        &      64,492           \tabularnewline[0.1cm]
        $R^2$           & & 0.1031        &    0.1157         &  0.2866    \tabularnewline[0.1cm]
        \hline\hline
        
    	\noalign{\vskip0.1cm}
    	\multicolumn{5}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Notes:} This table reports the regression results from Equations (\ref{eqn:error}). Dependent variables are the inflation nowcast errors (Column (1)), the inflation forecast errors (Column (2)), and the gas price forecast errors (Column (3)). "Stock" indicates dummies for stock market participation. We control for time-fixed effects and survey respondents' demographic fixed effects, including gender, education, birth cohort, marriage status, region, homeownership, and income quintiles. Robust standard errors are reported in the parenthesis.  $^{***}$, $^{**}$, $^{*}$ denotes statistical significance at 1\%, 5\%, and 10\% levels respectively.}    \\ 
    	{\footnotesize \textit{Sources:} Authors' calculation.} 
	\end{tabularx}
    }
\end{table}

==> Tables/tab_forecast.tex <==
\begin{table}
    \centering
    \caption{Stock holding and price forecasts} \label{tab:forecast}
    \small
    \centering
    \vspace{0.3cm}
	\noindent\resizebox{1.0\textwidth}{!}{
	\begin{tabularx}{\textwidth}{ll>{\centering}p{2.5cm}>{\centering}p{2.5cm}>{\centering}p{2.5cm}>{\centering}p{2.5cm}}
        \hline\hline
        \noalign{\vskip0.1cm}
                        & & \multicolumn{2}{c}{\textbf{Inflation}}   & \multicolumn{2}{c}{\textbf{Gas price}} \tabularnewline
        Dependent variable 
        &  & (1) 1-year & (2) 5-year & (3) 1-year & (4) 5-year \tabularnewline[0.1cm]
        \hline 
    	\noalign{\vskip0.1cm}
        Stock ($\beta$)  & & -0.332$^{***}$  & -0.236$^{***}$ & -0.078 & 1.290$^{***}$ \tabularnewline
                    & & (0.030)     &  (0.023) & (0.246) & (0.305)  \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        Time FE          & & Y & Y & Y & Y   \tabularnewline[0.1cm]
        Demographics FE  & & Y & Y & Y & Y    \tabularnewline[0.1cm]
        Number of obs.   & & 109,001  & 107,716 & 77,279 & 96,250  \tabularnewline[0.1cm]
        Adj. $R^2$       & & 0.0605 & 0.0258   &  0.0632   & 0.0578 \tabularnewline[0.1cm]
        \hline\hline
        
    	\noalign{\vskip0.1cm}
    	\multicolumn{6}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Notes:} This table reports the regression results from Equations (\ref{eqn:error}). Dependent variables are 1- and 5-year inflation and gas price forecasts. ``Stock'' indicates dummies for stock market participation. We control for time-fixed effects and survey respondents' demographic fixed effects, including gender, education, birth cohort, marriage status, region, homeownership, and income quintiles. Robust standard errors are reported in the parenthesis.  $^{***}$, $^{**}$, $^{*}$ denotes statistical significance at 1\%, 5\%, and 10\% levels respectively.}    \\ 
    	\multicolumn{6}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Sources:} Authors' calculation.} 
	\end{tabularx}
    }
\end{table}

==> Tables/tab_shock_old.tex <==
\begin{table}[ht!]
    \centering
    \caption{Sensitivity of households' expectations to macroeconomic shocks} \label{tab:shock}
    \small
    \centering
    \vspace{0.3cm}
	\noindent\resizebox{1.0\textwidth}{!}{
	\begin{tabularx}{\textwidth}{ll>{\centering}p{3.5cm}>{\centering}p{3.5cm}>{\centering}p{3.5cm}}
        \hline\hline
        \noalign{\vskip0.1cm}
        Macroeconomic shocks &  & (1) Inflation & (2) Business conditions & (3) Sentiment \tabularnewline[0.1cm]
        \hline 
        \noalign{\vskip0.1cm}
        \multicolumn{5}{l}{\textbf{\textit{Panel A. Fed information shocks}}} \tabularnewline
        \noalign{\vskip0.1cm}
        $\text{\emph{Stock}} \times \text{\emph{Shock}}_t$ ($\beta_1$)  
                 & &  0.065$^{***}$ &  0.072$^{***}$  &   1.000$^{***}$  \tabularnewline
                 & &     (0.016)    &    (0.008)      &    (0.147)          \tabularnewline[0.1cm]
        $\text{\emph{non-Stock}} \times \text{\emph{Shock}}_t$ ($\beta_2$)     
                 & &  0.101$^{***}$ &  0.045$^{***}$ &   0.515$^{***}$       \tabularnewline
                 & &     (0.025)    &   (0.010)       &    (0.186)   \tabularnewline[0.1cm]
        \noalign{\vskip0.1cm}
        \hline 
        \noalign{\vskip0.1cm}
        F-test: $\beta_1 = \beta_2$ & & 1.52         & 4.28$^{**}$  &  4.17$^{**}$ \tabularnewline[0.1cm]
        Number of obs.              & & 99,921       &      101,132    &  110,114      \tabularnewline[0.1cm]
        $R^2$                       & & 0.0262        &    0.0274       &  0.0765     \tabularnewline[0.1cm]
        \noalign{\vskip0.1cm}
        \hline 
        
        \noalign{\vskip0.1cm}
        \multicolumn{5}{l}{\textbf{\textit{Panel B. TFP news shocks}}} \tabularnewline
        \noalign{\vskip0.1cm}
        $\text{\emph{Stock}} \times \text{\emph{Shock}}_t$ ($\beta_1$)  
                 & &   -0.044$^{*}$ &  0.162$^{***}$  &   3.167$^{***}$  \tabularnewline
                 & &     (0.024)    &    (0.013)      &    (0.242)          \tabularnewline[0.1cm]
        $\text{\emph{non-Stock}} \times \text{\emph{Shock}}_t$ ($\beta_2$)     
                 & & -0.003         &  0.187$^{***}$ &   2.559$^{***}$       \tabularnewline
                 & &     (0.035)    &   (0.016)       &    (0.275)   \tabularnewline[0.1cm]
        \noalign{\vskip0.1cm}
        \hline 
        \noalign{\vskip0.1cm}
        F-test: $\beta_1 = \beta_2$ & & 0.93   &     1.6          &  2.78$^{*}$ \tabularnewline[0.1cm]
        Number of obs.              & & 45,934       &     47,868      &  51,330      \tabularnewline[0.1cm]
        $R^2$                       & & 0.0259        &    0.0316       &  0.0878     \tabularnewline[0.1cm]
        \noalign{\vskip0.1cm}

        \hline 
        
        \noalign{\vskip0.1cm}
        \multicolumn{5}{l}{\textbf{\textit{Panel C. Fed reaction to news}}} \tabularnewline
        \noalign{\vskip0.1cm}
        $\text{\emph{Stock}} \times \text{\emph{Shock}}_t$ ($\beta_1$)  
                 & &   0.134$^{*}$ &  0.188$^{***}$  &   3.127$^{***}$  \tabularnewline
                 & &     (0.020)    &    (0.008)      &    (0.163)          \tabularnewline[0.1cm]
        $\text{\emph{non-Stock}} \times \text{\emph{Shock}}_t$ ($\beta_2$)     
                 & &  0.071        &  0.144$^{***}$ &   2.534$^{***}$       \tabularnewline
                 & &     (0.035)    &   (0.011)       &    (0.216)   \tabularnewline[0.1cm]
        \noalign{\vskip0.1cm}
        \hline 
        \noalign{\vskip0.1cm}
        F-test: $\beta_1 = \beta_2$ & & 2.79$^{*}$   &     10.14$^{***}$          &  4.83$^{**}$ \tabularnewline[0.1cm]
        Number of obs.              & & 108,755       &     110.523      &  120,147      \tabularnewline[0.1cm]
        $R^2$                       & & 0.0285        &    0.0294       &  0.0768     \tabularnewline[0.1cm]
        \noalign{\vskip0.1cm}

        
        \hline\hline
        
        \noalign{\vskip0.1cm}
        \multicolumn{5}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Notes:} This table reports the regression results from Equations (\ref{eqn:shock}). The dependent variables are 1-year ahead inflation expectations (Column (1)), business conditions outlook (Column (2)), and index of consumer sentiment (Column (3)). ``Stock'' indicates dummies for stock market participation. ``Shock'' denotes Fed information shock (Panel A), TFP news shock (Panel B), and Fed reaction to news (Panel C). The coefficients reported are based on a \emph{1-std.dev.} increase in each type of shock. We control for survey respondents' demographic fixed effects, including gender, education, birth cohort, marriage status, region, homeownership, and income quintiles. Robust standard errors are reported in the parenthesis.  $^{***}$, $^{**}$, $^{*}$ denotes statistical significance at 1\%, 5\%, and 10\% levels respectively.}   \\ 
        {\footnotesize \textit{Sources:} Authors' calculation.} 
	\end{tabularx}
    }
\end{table}

==> Tables/tab_uncertain_old.tex <==
\begin{table}
    \centering
    \caption{Sensitivity of attention to changes in economic policy uncertainty} \label{tab:uncertain}
    \small
    \centering
    \vspace{0.3cm}
	\noindent\resizebox{0.95\textwidth}{!}{
	\begin{tabularx}{\textwidth}{ll>{\centering}p{3.5cm}>{\centering}p{3.5cm}>{\centering}p{3.5cm}}
        \hline\hline
        \noalign{\vskip0.1cm}
        Dependent variable &  & (1) Attention & (2) Inflation & (3) Gas price \tabularnewline[0.1cm]
        \hline 
    	\noalign{\vskip0.1cm}
        \multicolumn{4}{l}{\textbf{\textit{Panel A: News-based policy uncertainty}}} \tabularnewline[0.1cm]
        $\text{\emph{Stock}} \times \text{\emph{Uncertainty}}_t$ ($\beta_1$)  
                 & &  0.059$^{***}$ &  0.089$^{***}$  &   -1.839$^{***}$  \tabularnewline
                 & &     (0.002)    &    (0.012)      &    (0.063)          \tabularnewline[0.1cm]
        $\text{\emph{non-Stock}} \times \text{\emph{Uncertainty}}_t$ ($\beta_2$)     
                 & &  0.025$^{***}$ &   0.211$^{***}$ &   -1.899$^{***}$       \tabularnewline
                 & &     (0.002)    &   (0.015)       &    (0.071)   \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        F-test: $\beta_1 = \beta_2$ & & 486.72$^{***}$ & 123.38$^{***}$  &  1.30 \tabularnewline[0.1cm]
        Number of obs.              & & 109,001       &      109,001    &  64,492      \tabularnewline[0.1cm]
        $R^2$                       & & 0.0781        &    0.0305       &  0.0158     \tabularnewline[0.1cm]

        \hline 
        \noalign{\vskip0.1cm}
        \multicolumn{4}{l}{\textbf{\textit{Panel B: Market-Based monetary policy uncertainty}}} \tabularnewline[0.1cm]
        $\text{\emph{Stock}} \times \text{\emph{Uncertainty}}_t$ ($\beta_1$)  
                 & &  0.030$^{***}$ &  0.250$^{***}$  &   4.765$^{***}$  \tabularnewline
                 & &     (0.002)    &    (0.012)      &    (0.120)          \tabularnewline[0.1cm]
        $\text{\emph{non-Stock}} \times \text{\emph{Uncertainty}}_t$ ($\beta_2$)     
                 & &  -0.004$^{***}$ &   0.299$^{***}$ &   4.889$^{***}$       \tabularnewline
                 & &     (0.002)    &   (0.013)       &    (0.135)   \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        F-test: $\beta_1 = \beta_2$ & & 694.51$^{***}$ & 24.42$^{***}$  &  1.43 \tabularnewline[0.1cm]
        Number of obs.              & & 120,147       &      108,755    &  69,526      \tabularnewline[0.1cm]
        $R^2$                       & & 0.0773        &    0.0351       &  0.0400     \tabularnewline[0.1cm]
        
        \hline 
        \noalign{\vskip0.1cm}
        \multicolumn{4}{l}{\textbf{\textit{Panel C: Macro uncertainty}}} \tabularnewline[0.1cm]
        $\text{\emph{Stock}} \times \text{\emph{Uncertainty}}_t$ ($\beta_1$)  
                 & &  0.047$^{***}$ &  0.540$^{***}$  &   3.190$^{***}$  \tabularnewline
                 & &     (0.001)    &    (0.014)      &    (0.084)          \tabularnewline[0.1cm]
        $\text{\emph{non-Stock}} \times \text{\emph{Uncertainty}}_t$ ($\beta_2$)     
                 & &  0.032$^{***}$ &   0.589$^{***}$ &   3.24$^{***}$       \tabularnewline
                 & &     (0.001)    &   (0.014)       &    (0.087)   \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        F-test: $\beta_1 = \beta_2$ & & 666.42$^{***}$ & 132.46$^{***}$  &  2.41 \tabularnewline[0.1cm]
        Number of obs.              & & 120,147       &      108,755    &  69,526      \tabularnewline[0.1cm]
        $R^2$                       & & 0.0824        &    0.0546       &  0.0268     \tabularnewline[0.1cm]

        \hline 
        \noalign{\vskip0.1cm}
        \multicolumn{4}{l}{\textbf{\textit{Panel D: Financial uncertainty}}} \tabularnewline[0.1cm]
        $\text{\emph{Stock}} \times \text{\emph{Uncertainty}}_t$ ($\beta_1$)  
                 & &  0.028$^{***}$ &  0.238$^{***}$  &   2.325$^{***}$  \tabularnewline
                 & &     (0.001)    &    (0.010)      &    (0.066)          \tabularnewline[0.1cm]
        $\text{\emph{non-Stock}} \times \text{\emph{Uncertainty}}_t$ ($\beta_2$)     
                 & &  0.011$^{***}$ &   0.270$^{***}$ &   2.400$^{***}$       \tabularnewline
                 & &     (0.001)    &   (0.010)       &    (0.071)   \tabularnewline[0.1cm]
                    \hline 
        \noalign{\vskip0.1cm}
        F-test: $\beta_1 = \beta_2$ & & 801.73$^{***}$ & 54.17$^{***}$  &  3.72$^{*}$ \tabularnewline[0.1cm]
        Number of obs.              & & 120,147       &      108,755    &  69,526       \tabularnewline[0.1cm]
        $R^2$                       & & 0.0796        &    0.0305       &  0.0198     \tabularnewline[0.1cm]
        
        \hline\hline
        
        \noalign{\vskip0.1cm}
        \multicolumn{5}{p{\dimexpr\linewidth-2\tabcolsep-2\arrayrulewidth}}{\footnotesize \textit{Notes:} This table reports the regression results from Equations (\ref{eqn:uncertain}). Dependent variables are \emph{Attention} (Column (1)), the inflation forecast errors (Column (2)), and the gas price forecast errors (Column (3)). ``Stock'' indicates dummies for stock market participation. ``Uncertainty'' denotes news-based economic policy uncertainty index (Panel A), market-based monetary policy uncertainty (Panel B), macro uncertainty (Panel C), and financial uncertainty (Panel D) respectively. The coefficients reported are based on a \emph{1-std.dev.} increase in the index. We control for survey respondents' demographic fixed effects, including gender, education, birth cohort, marriage status, region, homeownership, and income quintiles. Robust standard errors are reported in the parenthesis.  $^{***}$, $^{**}$, $^{*}$ denotes statistical significance at 1\%, 5\%, and 10\% levels respectively.}   \\ 
    	{\footnotesize \textit{Sources:} Authors' calculation.} 
	\end{tabularx}
    }
\end{table}

==> literature.tex <==

@article{10.1093/rfs/hhy089,
    author = {Vestman, Roine},
    title = "{Limited Stock Market Participation Among Renters and Homeowners}",
    journal = {The Review of Financial Studies},
    volume = {32},
    number = {4},
    pages = {1494-1535},
    year = {2018},
    month = {08},
    abstract = "{The stock market participation rate among homeowners is twice as high as among renters. This paper builds a life-cycle portfolio choice model with endogenous housing tenure choice. A stylized form of preference heterogeneity generates a substantial difference in participation rates. A majority of households have a large savings motive and choose to be homeowners and participate. A minority of households have a small savings motive and find it less worthwhile to participate. Fewer of these households become homeowners. Difference-in-difference regressions on panel data do not find evidence of a crowding-out effect of homeownership on participation, supporting the message that preference heterogeneity matters.Received January 25, 2017; editorial decision March 21, 2018 by Editor Wei Jiang. Authors have furnished an Online Appendix, which is available on the Oxford University Press Web site next to the link to the final published paper online.}",
    issn = {0893-9454},
    doi = {10.1093/rfs/hhy089},
    url = {https://doi.org/10.1093/rfs/hhy089},
    eprint = {https://academic.oup.com/rfs/article-pdf/32/4/1494/28021872/hhy089.pdf},
}

@article{10.1093/rfs/hhz041,
    author = {Das, Sreyoshi and Kuhnen, Camelia M and Nagel, Stefan},
    title = "{Socioeconomic Status and Macroeconomic Expectations}",
    journal = {The Review of Financial Studies},
    volume = {33},
    number = {1},
    pages = {395-432},
    year = {2019},
    month = {03},
    abstract = "{We show that individuals’ macroeconomic expectations are influenced by their socioeconomic status (SES). People with higher income or higher education are more optimistic about future macroeconomic developments, including business conditions, the national unemployment rate, and stock market returns. The spread in beliefs between high- and low-SES individuals diminishes significantly during recessions. A comparison with professional forecasters and historical data reveals that the beliefs wedge reflects excessive pessimism on the part of low-SES individuals. SES-driven expectations help explain why higher-SES individuals are more inclined to invest in the stock market and more likely to consider purchasing homes, durable goods, or cars.Received November 13, 2017; editorial decision February 12, 2019 by Editor Wei Jiang. Authors have furnished an Internet Appendix, which is available on the Oxford University Press Web site next to the link to the final published paper online.}",
    issn = {0893-9454},
    doi = {10.1093/rfs/hhz041},
    url = {https://doi.org/10.1093/rfs/hhz041},
    eprint = {https://academic.oup.com/rfs/article-pdf/33/1/395/32742335/hhz041.pdf},
}

@article{10.1093/rfs/hhaa116,
    author = {Cieslak, Anna and Vissing-Jorgensen, Annette},
    title = "{The Economics of the Fed Put}",
    journal = {The Review of Financial Studies},
    volume = {34},
    number = {9},
    pages = {4045-4089},
    year = {2020},
    month = {10},
    abstract = "{Since the mid-1990s, negative stock returns comove with downgrades to the Fed’s growth expectations and predict policy accommodations. Textual analysis of FOMC documents reveals that policy makers pay attention to the stock market. The primary mechanism is their concern with the consumption wealth effect, with a secondary role for the market predicting the economy. We find little evidence of the Fed overreacting to the market in an ex post sense (reacting beyond the market’s effect on growth expectations). Although policy makers are aware that the Fed put could induce risk-taking, moral hazard considerations appear not to significantly affect their decision-making ex ante.}",
    issn = {0893-9454},
    doi = {10.1093/rfs/hhaa116},
    url = {https://doi.org/10.1093/rfs/hhaa116},
    eprint = {https://academic.oup.com/rfs/article-pdf/34/9/4045/39831090/hhaa116.pdf},
}


@article{ehrmann2017consumers,
  title={Consumers' Attitudes and Their Inflation Expectations},
  author={Ehrmann, Michael and Pfajfar, Damjan and Santoro, Emiliano and others},
  journal={International Journal of Central Banking},
  volume={13},
  number={1},
  pages={225--259},
  year={2017},
  publisher={International Journal of Central Banking}
}

@article{jurado2015measuring,
  title={Measuring uncertainty},
  author={Jurado, Kyle and Ludvigson, Sydney C and Ng, Serena},
  journal={American Economic Review},
  volume={105},
  number={3},
  pages={1177--1216},
  year={2015}
}

@article{ludvigson2021uncertainty,
  title={Uncertainty and business cycles: exogenous impulse or endogenous response?},
  author={Ludvigson, Sydney C and Ma, Sai and Ng, Serena},
  journal={American Economic Journal: Macroeconomics},
  volume={13},
  number={4},
  pages={369--410},
  year={2021}
}

@techreport{bauer2022reassessment,
  title={A reassessment of monetary policy surprises and high-frequency identification},
  author={Bauer, Michael D and Swanson, Eric T},
  year={2022},
  institution={National Bureau of Economic Research}
}

@article{bauer2022market,
  title={Market-based monetary policy uncertainty},
  author={Bauer, Michael D and Lakdawala, Aeimit and Mueller, Philippe},
  journal={The Economic Journal},
  volume={132},
  number={644},
  pages={1290--1308},
  year={2022},
  publisher={Oxford University Press}
}

/******* Theory papers ******************************************/

@article{zhang2017rational,
  title={Rational inattention in uncertain business cycles},
  author={Zhang, Fang},
  journal={Journal of Money, Credit and Banking},
  volume={49},
  number={1},
  pages={215--253},
  year={2017},
  publisher={Wiley Online Library}
}


@article{gaballo2016rational,
  title={Rational inattention to news: The perils of forward guidance},
  author={Gaballo, Gaetano},
  journal={American Economic Journal: Macroeconomics},
  volume={8},
  number={1},
  pages={42--97},
  year={2016}
}


@article{andrei2022economic,
  title={Economic Uncertainty and Investor Attention},
  author={Andrei, Daniel and Friedman, Henry and Ozel, N Bugra},
  year={2022}
}

@article{huang2007rational,
  title={Rational inattention and portfolio selection},
  author={Huang, Lixin and Liu, Hong},
  journal={The Journal of Finance},
  volume={62},
  number={4},
  pages={1999--2040},
  year={2007},
  publisher={Wiley Online Library}
}
